Computer-assisted validation of the existence of periodic orbit in the Brusselator system

We investigate the Brusselator system with diffusion and Dirichlet boundary conditions on one dimensional space interval. Our proof demonstrates that, for certain parameter values, a periodic orbit exists. This proof is computer-assisted and rooted in the rigorous integration of partial differential equations. Additionally, we present the evidence of the occurrence of period-doubling bifurcation.

==> parts/introductionForRevievs.tex <==

\section{Introduction}
In this paper, we study the dynamics of the Brusselator system with diffusion, described by the following initial and boundary value problem consisting of two mutually coupled partial differential equations.
\begin{equation}\label{eq:BrusselatorPDE}
\begin{cases}
 u_t = d_1  u_{xx}- (B+1)u +u^2v + A \sin(x) \;  \text{for}\; (x,t)\in (0,\pi)\times(0,\infty),\\
 v_t = d_2 v_{xx} + Bu - u^2v  \;  \text{for}\; (x,t)\in (0,\pi)\times(0,\infty),\\
u(t,x)= v(t,x) = 0\; \text{for}\; (x,t)\in \{0,\pi\} \times (0,\infty),
\\u(0,x) = u^0(x),\ v(0,x) = v^0(x)\ \textrm{for}\ x\in(0,\pi).
\end{cases}
\end{equation}
The system models autocatalytic reactions in form
\begin{align*}
    &A \rightarrow u,
    \\&2u + v \rightarrow 3u,
     \\&B + u \rightarrow v + D,
     \\&u \rightarrow E.
\end{align*}
The coefficients $A,B$ in the system are given and they correspond to densities of the substances $A$ and $B$ in the above reactions. The unknown functions $u(t,x)$ and $v(t,x)$ describe the densities of two substances which we also denote by $u$ and $v.$ The system \eqref{eq:BrusselatorPDE} is an extension of the planar Brusselator ODE \eqref{eq:BrusselatorODE} where the substances $u$ and $v$ are homogeneously spread in the domain.
The terms $u_{xx}$ and $v_{xx}$ represent the diffusion of substances. The coefficients
$d_1,d_2$ are the corresponding diffusion rates.

If we drop the diffusion and the dependence on the variable $x$ in the term $A\sin(x)$ from the system \eqref{eq:BrusselatorPDE}, we obtain the following planar ODE
\begin{equation}\label{eq:BrusselatorODE}
	\begin{cases}
		u' = - (B+1)u +u^2v + A  \ \   \text{for}\ \  t\in \R,\\
		v' = Bu - u^2v  \ \   \text{for}\ \  t\in \R.
	\end{cases}
\end{equation}
The planarity of the above system implies that the invariant sets consist of fixed points, periodic orbits, and heteroclinic connections between them. In fact, it is known that in \eqref{eq:BrusselatorODE}, \textcolor{blue}{there can exist an attracting periodic orbit that arises via the Hopf bifurcation} \cite[Theorem 3]{HopfBifurcationGeneralBrusselator}.
The analytical results about the Brusselator system of PDEs with diffusion are limited.
In the article \cite{YouBrusselatorAttractor} the existence of the global attractor for the Brusselator system on the 3-dimensional domain is proved. \textcolor{blue}{While this global attractor is known to exist, the question about its structure, which pertains to the understanding of the problem dynamics, remains unanswered}. Some partial analytical results about the dynamics are available for Neumann boundary conditions, where the homogeneous steady state is known from the solutions of the corresponding ODE \eqref{eq:BrusselatorODE}. In this case, one can linearize the system of PDEs in its vicinity. Such results are available for example in \cite{BROWN19951713} and \cite{StabilityPeñaBegoña}.
The case with Dirichlet conditions, which we consider, appears to be much more challenging. In \cite{AUCHMUTY1975323}, the stability analysis of the steady state was carried out for Dirichlet \textcolor{blue}{non-homogeneous conditions. In such case there exists a nonzero homogeneous steady state}. However, this type of analysis is not possible for the problem we are dealing with, as the homogeneous steady state does not exist (it would have to be equal to zero). Based on numerical observations, the system  \eqref{eq:BrusselatorPDE} possesses a periodic orbit for some range of parameters $d_1, d_2, A, B$. We anticipate that this periodic orbit arises from a mechanism similar to the one known for the planar ODE \eqref{eq:BrusselatorODE}, namely through a Hopf bifurcation.

We deal with the apparent impossibility of obtaining purely analytical results on the periodic orbit existence by using the computer assisted techniques.

Specifically, we perform a computer-assisted proof of the following theorem.
\begin{theorem} \label{th:BrusselatorPeriodicOrbit}
For the parameters $d_1 = 0.2$, $d_2 = 0.02$, $A = 1$, and $B= 2$, the Brusselator system has a time-periodic orbit.
%Moreover this periodic orbit is symmetric with respect to line $y = \frac{\pi}{2}$.
\end{theorem}
\begin{figure}[h]
    \includegraphics[width=0.9\linewidth, height=6cm]
    {Pictures/fig1.pdf}
\label{fig:image3}
\caption{The numerical approximation of the time-periodic orbit obtained in Theorem \ref{th:BrusselatorPeriodicOrbit}.
Blue and orange surfaces
correspond to plots of $u(t,x)$ and $v(t,x)$ respectively.
}
\end{figure}

\textcolor{blue}{It is worth noting that while numerical simulations suggest that this orbit from Theorem \ref{th:BrusselatorPeriodicOrbit} appears to be attracting, it has not been rigorously proven to be so.}


The results on the existence of periodic orbit for the Brusselator were also obtained recently, together with the proof of the Hopf bifurcation, also using the computer assisted techniques, in the paper \cite{ArioliBrusselator}. The approach employed there is based on the Newton--Kantorovich method. The author demonstrates that a specific Newton-type operator has a fixed point, enabling him to establish the existence of a periodic orbit. This class of methods has been successfully applied for many problems governed by PDEs (see for example \cite{NSArioliHopf,NSLessBreden,EllipticSurvay,ElipticUnboundedPlum}).
The monograph \cite{ValidationBookPlum} contains detailed description and up to date overview of these methods together with numerous applications.
 In our  proof of Theorem \ref{th:BrusselatorPeriodicOrbit} we are using different method.  Namely, our approach   is based on the algorithm of rigorous forward integration of the dissipative systems.
This method was developed in articles  \cite{ZPKuramotoII,ZPKuramotoIII} and applied there for the Kuramoto--Shivasinski equation.
Similarly, as in the above works, we express the solution in terms of the Fourier series.
Specifically, as the solutions $u(t,x)$ and $v(t,x)$ satisfy the Dirichlet boundary conditions on $[0,\pi]$, they are represented as the sum of sine Fourier series
\begin{equation}\label{eq:decomposion}
u(t,x) = \sum_{i=1}^\infty u_i(t)\sin(i x),\quad
v(t,x) = \sum_{i=1}^\infty v_i(t)\sin(i x).
\end{equation}
The ability to work with all Fourier coefficients facilitates a straightforward and efficient integration of the Brusselator system. It is noteworthy, however, that in Theorem \ref{th:Arioli}, we obtain the same periodic orbit as in \cite{ArioliBrusselator}, cross-validating the accuracy of the two distinct methods.
Other approaches of representing the solution are also possible. In the work \cite{FEMPiotrek} the solution to the Burgers equation was represented by the first order finite element basis together with the estimates on the norms in the Sobolev spaces.

\textcolor{blue}{Note that the constant term $A$ from the ODE \eqref{eq:BrusselatorODE} has been replaced by the term $A\sin(x)$ in our PDE extension of the Brusselator system. In principle, we could consider the PDE version of the problem with the constant term $A$, that is the following system 
\begin{equation}\label{eq:BrusselatorPDEILL}
\begin{cases}
 u_t = d_1  u_{xx}- (B+1)u +u^2v + A  \;  \text{for}\; (x,t)\in (0,\pi)\times(0,\infty),\\
 v_t = d_2 v_{xx} + Bu - u^2v  \;  \text{for}\; (x,t)\in (0,\pi)\times(0,\infty),\\
u(t,x)= v(t,x) = 0\; \text{for}\; (x,t)\in \{0,\pi\} \times (0,\infty),
\\u(0,x) = u^0(x),\ v(0,x) = v^0(x)\ \textrm{for}\ x\in(0,\pi).
\end{cases}
\end{equation}
In such a case, we observe that $u_{xx}(t,x) = -\frac{A}{d_1}\not = 0$ for the boundary points  $x\in \{0,\pi\}.$ and for every $t\in\mathbb{R}^+,$ which means that compatibly conditions are not met. 
Let us represent $u$ in term of the sine Fourier series \eqref{eq:decomposion}. Assume that the series $\sum_{i=1}^\infty |u_i(t)|i^2$ is convergent.  Then, we can differentiate the Fourier series  twice, and we obtain 
\begin{equation*}
    u_{xx}(t,x) = \sum_{i=1}^\infty -u_i(t)i^2\sin(i x)
\end{equation*}
Therefore $u_{xx}(t,x) = 0$ for $x\in\{0,\pi\},$ which is not true, and hence, by contradiction, the series  $\sum_{i=1}^\infty |u_i(t)|i^2$ has to diverge.   Therefore, the Fourier series cannot converge to the solution fast. This unwelcome effect does not occur when we consider term $A\sin(x)$ instead of $A$ in the system \eqref{eq:BrusselatorPDE}, because the function $Asin(x)$ on $[0,\pi]$ is a restriction of a smooth, odd and $2\pi$ periodic function.
} 


The novelty of the present paper is the proof of the periodic orbit existence for the Brusselator systems using the rigorous forward integration techniques. This integration algorithm is, according to our knowledge, applied by us \textcolor{blue}{for the first time for a system of PDEs}: in our case two mutually coupled nonlinear parabolic PDEs with polynomials of order $3$ in the nonlinear term.  We  underline that the rigorous integration scheme which we use is the same as in  \cite{ZPKuramotoII, ZPKuramotoIII}, where it was used for the Kuramoto--Sivashinski equation with odd-periodic boundary conditions. We show its applicability for the problem with higher degree of nonlinearity: is our case the two equations of the system are coupled through the cubic term, while the nonlinearity in the Kuramoto--Sivashinsky equation is quadratic. The key concept which makes it possible for the integration scheme to work is the same in our case as in  \cite{ZPKuramotoII, ZPKuramotoIII}. Namely, the dissipativity of the leading linear operator together with appropriate a priori estimates for the nonlinearity, which is of lower order, allow the linear  terms to dominate over the nonlinear ones at appropriately high modes in  the Fourier expansion. This allows us to treat the tail of the Fourier expansion uniformly, by controlling a polynomial decay of the coefficients in every time step, cf. Lemma~\ref{lem:whyItWorks}.  Our techniques hold potential for wider applicability. To this end, in Section \ref{sec:algebra}, we establish estimates on the convolution of sine and cosine Fourier series, which can be utilized to calculate nonlinear terms for a general dissipative system with polynomial nonlinearities in one spatial dimension. These estimates are a crucial component in rigorous integration algorithms for such systems.
    A further innovation is that in our theoretical results, which ensure the validity of the algorithm, we don't require the use of Galerkin projections of the solution\textcolor{red}{, as it is demonstrated in Lemma \ref{lemma:enclosure} below}. Instead, we work directly with the solution of the PDE system \textcolor{blue}{on the level of abstract theorems as can be seen in Sections \ref{sec:AlgorithmIntegration} and \ref{sec:comAssisedProof}}. This simplifies our assumptions \textcolor{red}{see  (A1)--(A2) and (B1)--(B3) below,} and hence it makes the results more accessible to the dissipative PDE community. Additionally, we examine the limitations of our algorithm for PDEs with nonlinearities that do not meet the compatibility condition on the boundary: \textcolor{blue}{  this is the case even with the constant $A$ in place of  $A\sin(x)$ in the equation for $u_t$ in the Brusselator system \eqref{eq:BrusselatorPDE}. We illustrate this issue by considering the problem governed by the diffusive logistic equation \eqref{eq:logisticEquation} as an example.}

 In Section \ref{sec:numerical}, we observe that for a sufficiently large parameter $B$, the system exhibits slow-fast behavior, as expected for the Brusselator system and known in the ODE case. This effect is stronger for higher Fourier modes. To demonstrate this, we establish the existence of periodic orbits for parameters $d_1 = 0.2,\;d_1 = 0.02,\;A=1,\;B=2+\frac{i}{10}$ for $i\in{0,\dots,11}$. Figures \ref{fig:OrbitsPlots1} and \ref{fig:OrbitsPlots2} show that some of these orbits exhibit slow-fast behavior.

 In \cite{ArioliBrusselator} Arioli observed a period doubling bifurcation, a phenomenon that cannot occur in the planar ODE \eqref{eq:BrusselatorODE}. Thus, the dynamics of \eqref{eq:BrusselatorPDE} is expected to be more complicated than that of the planar ODE \eqref{eq:BrusselatorODE}. Although we do not rigorously prove the bifurcation, we also show that the minimal period of the found orbits approximately doubles with a small increase in the parameter $B$, as seen in Theorem \ref{th:podwojenieOkresu}. \textcolor{blue}{In this range of parameter $B$ there should  also exist one unstable orbit with the period that is not doubled. To prove the existence of this kind of orbit we could use the rigorous solver for the Brusselator system together with the concept of $h$-sets and covering relations (see for example \cite[Section 2.1]{KuramotoAutomaticDiff} and \cite[Section 10.2]{ZPKuramotoIII}). Such approach has been successfully used to prove the existence of unstable periodic orbits before \cite[Theorem 45, Theorem 46]{ZPKuramotoIII}).
}

Other nontrivial dynamics of the Brusselator system, such as the existence of 2-dimensional attracting tori and chaos, were numerically investigated in \cite{BrusselatorChaosAnd2DTori}. Our numerical observations support the existence of 2-dimensional attracting tori for small diffusion parameters, although a rigorous proof of their existence remains an open problem. There are many avenues for further research on this topic. Numerical simulations indicate that the periodic orbit established in Theorem \ref{th:BrusselatorPeriodicOrbit} is attracting. However, providing a rigorous computer-assisted proof of this observation is challenging, as it requires a rigorous $C^1$ calculation, i.e. the integration of the variational equation for the Brusselator system.


The structure of the article is as follows.
In  Section \ref{sec:AlgorithmIntegration} we describe the algorithm of rigorous integration for dissipative equations. In Section \ref{sec:comAssisedProof} we describe the computer assisted proof of  Theorem
\ref{th:BrusselatorPeriodicOrbit}.
 In Section \ref{sec:crossing}, we address the algorithm for computing the Poincaré map and prove Theorem \ref{th:PoincareFixedPoint}, which pertains to the fixed point of this map which corresponds to the periodic orbit of the system. In the remaining part of Section \ref{sec:comAssisedProof} we describe the validation of the assumptions of this theorem for the Brusselator system.
 Section \ref{sec:numerical} contains numerical and rigorous results for various parameters of the Brusselator system.
Finally, in Section \ref{sec:algebra}, we provide results on the algebra of infinite series, which is utilized in the algorithms.

\textcolor{blue}{The code which was used in computer assisted proofs is published at GitHub \cite{Code} and based on  CAPD library \cite{CAPD,CAPDArticle}.
}










\begin{comment}

Brusselator system in ODE case has a periodic orbit for some parameters which arises from Hopf biffurcation of stationary point.
In this paper we are proving that periodic orbit also exists for the system with diffusion and Dirichlet boundary conditions. Prove is computer assisted.
\end{comment}






==> parts/poincareMap.tex <==


\section{Poincare map}
Now we will give some results concerning continuity of Poincare map.



==> parts/problemDef.tex <==

\section{Problem definition and main results}

As $u(t,x) ,v(t,x)$ are satisfying Dirichlet boundary condition on interval $[0,\pi]$ we can write them in Fourier base
\begin{equation}\label{eq:decomposion}
u(t,x) = \sum_{i=1}^\infty u_i(t)\sin(i x),\quad
v(t,x) = \sum_{i=1}^\infty v_i(t)\sin(i x).
\end{equation}







